Pleasant Imperative Program Proofs with GallinaC

Even with the increase of popularity of functional programming, imperative programming remains a key programming paradigm, especially for programs operating at lower levels of abstraction. When such software offers key components of a Trusted Computing Base (TCB), e.g. an operating system kernel, it becomes desirable to provide mathematical correctness proofs. However, current real-world imperative programming languages possess "expressive", i.e. overly permissive, semantics. Thus, producing correctness proofs of such programs becomes tedious and error-prone, requiring to take care of numerous "administrative" details. Ideally, a proof-oriented imperative language should feature well-behaved semantics while allowing imperative idioms. To obtain a high-degree of confidence in the correctness of such a language, its tools should be developed inside a proof-assistant such that program proofs are machine checked. We present GallinaC, a shallow embedding of a Turing-complete imperative language directly inside the functional programming language of the Rocq proof assistant, Gallina. In particular, it features a truly generic and unbounded while loop. Having a functional core means proofs about GallinaC programs may use the same tactics as proofs about pure functional ones. Work on GallinaC is still under progress, but we present first promising results. A prototype implementation has shown the viability of GallinaC with the correctness proof of a list reversal procedure for linked-lists of unknown size. We currently focus on the forward simulation between the GallinaC intermediate representation (IR) and Cminor, the entry language of the CompCert back-end.

==> eptcsdata.tex <==
\providecommand{\firstpage}{24}
\providecommand{\publicationstatus}{Andrei Arusoaie, Hora\c{t}iu Cheval, Radu Iosif: FROM 2025\\
EPTCS 427, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.427.2}{10.4204/EPTCS.427.2}}

